SuperUDF: Self-supervised UDF Estimation for Surface Reconstruction

Learning-based surface reconstruction based on unsigned distance functions (UDF) has many advantages such as handling open surfaces. We propose SuperUDF, a self-supervised UDF learning which exploits a learned geometry prior for efficient training and a novel regularization for robustness to sparse sampling. The core idea of SuperUDF draws inspiration from the classical surface approximation operator of locally optimal projection (LOP). The key insight is that if the UDF is estimated correctly, the 3D points should be locally projected onto the underlying surface following the gradient of the UDF. Based on that, a number of inductive biases on UDF geometry and a pre-learned geometry prior are devised to learn UDF estimation efficiently. A novel regularization loss is proposed to make SuperUDF robust to sparse sampling. Furthermore, we also contribute a learning-based mesh extraction from the estimated UDFs. Extensive evaluations demonstrate that SuperUDF outperforms the state of the arts on several public datasets in terms of both quality and efficiency. Code url is https://github.com/THHHomas/SuperUDF.

==> 0abstract.tex <==
\begin{abstract}
Learning-based surface reconstruction based on unsigned distance functions (UDF) has many advantages such as handling open surfaces. We propose SuperUDF, a self-supervised UDF learning which exploits a learned geometry prior for efficient training and a novel regularization for robustness to sparse sampling. The core idea of SuperUDF draws inspiration from the classical surface approximation
operator of locally optimal projection (LOP). The key insight is that if the UDF is estimated correctly, the 3D points should be locally projected onto the
underlying surface following the gradient of the UDF. Based on that, a number of inductive biases on UDF geometry and a pre-learned geometry prior are devised to learn UDF estimation efficiently. A novel regularization loss is proposed to make SuperUDF robust to sparse sampling. Furthermore, we also contribute a learning-based mesh extraction from the estimated UDFs. Extensive evaluations demonstrate that SuperUDF outperforms the state of the arts on several public datasets in terms of both quality and efficiency.

%extract iso-surface via elevating the UDF to SDF. We propose SuperUDF, a self-supervised learning method for UDF estimation,  The training of UDF estimation is self-supervised based on several inductive biases on UDF geometry. To ease the learning, we opt to estimate a projection flow of points onto the underlying surface as an approximation of UDF gradients. The UDF is obtained from the projection flow based on their duality. 

%Reconstructing clean surfaces from the raw scanned point clouds is a fundamental problem for many computer graphics and vision applications. Given the extra point normals, the classic Poisson surface reconstruction method can recover the missing geometry details by solving the Poisson equation. To remove the requirement of point normals, some signed distance functions (SDFs) based methods adopt neural networks with prior supervised knowledge to reconstruct the closed 3D surface. However, neither the point normals nor surface reconstruction supervision is easy to acquire in practice applications such as active mapping. We introduce SuperUDF, a neural network-based framework with unsigned distance functions (UDFs) that can learn any type of surface topology from raw 3D point clouds directly in a self-supervised fashion. A novel loss design is proposed to enable self-supervised training for UDFs estimation. Since no sign is given to distinguish the inner and outer for reconstruction, we then propose a neural network module to predict the relative sign of the vertex of the local grid. Note that the training only focuses on small surface geometry patches. It only requires a small, fixed set of clean shapes for all types of testing data. Since our method estimates UDPs and reconstructs the surface individually, which reduces the training difficulty, our framework can recover more fine-grained geometry details. To demonstrate the effectiveness of our method, we evaluate our method on ShapeNet, Garment, and ScanNet. Our self-supervised method can achieve XXXX\% improvement compared with state-of-the-art alternatives with more supervision.
%Learning implicit surface from 3D point cloud is an important task and has been highly demanded by many applications recently. Almost all the learning methods nowadays need 3D ground-truth during training. However, it is not only expensive but also limited because real world scene do not have 3D ground-truth. Thus, we develop an unsupervised method for surface reconstruction from point cloud which can be applied to watertight synthetic shape and non-watertight real world scene. We adopt UDF (unsiged distance function) rather than SDF (signed distance function) to represent the surface because SDF can only represent watertight surface and harder to learn than UDF. Our method consists of two parts, estimating UDF from point cloud and extracting surface from UDF. For the former part, we propose 
%a network to predict the shift from point around the surface to surface and propose a high effectiveness constraints to guide the UDF distribution around the surface mimicking the idea in Sphere Marching\cite{}. For the latter part, we modifying the Marching Cube\cite{} and predict the relative sign of the vertex of local cube rather absolute sign using a tiny neural network, thus generating a surface without orientation. In order to show the effectiveness of our method, we provide experiment result on ShapeNet, Garment and ScanNet. Our method achieve comparable result with the supervised method. Code will be released. 
\end{abstract}

==> figures/garment_result2.tex <==
\begin{figure} 
\centering
  \includegraphics[width=\columnwidth]{figures/images/garmet_result2.pdf}
  \caption{Visualized results of our method, traditional reconstruction methods PSR\cite{2013Poisson} and 3 deep method NDF\cite{2020ndf}, CAP\cite{capudf}, GIFS\cite{gifs} on garment dataset. Note that we provide the ground-truth normal as input for PSR as it requires.}
  \label{fig:garment_result2}
\end{figure}

==> figures/garment_result3.tex <==
\begin{figure} 
\centering
  \includegraphics[width=\columnwidth]{figures/images/garment_result3.pdf}
  \caption{Visualized results of our method, traditional reconstruction methods PSR\cite{2013Poisson} and 3 deep method NDF\cite{2020ndf}, CAP\cite{capudf}, GIFS\cite{gifs} on garment dataset. Note that we provide the ground-truth normal as input for PSR as it requires.}
  \label{fig:garment_result3}
\end{figure}

==> figures/main_result2.tex <==
\begin{figure*} 
\centering
  \includegraphics[width=2\columnwidth]{figures/images/main_result2}
  \caption{Visualized results of our method and 2 traditional reconstruction methods PSR and BPA.}
  \label{fig:main_result2}
\end{figure*}

==> figures/reg2.tex <==
\begin{figure}
\centering
  \includegraphics[width=0.8\columnwidth]{figures/images/reg2.pdf}
  \caption{The second regularization of $UDF$ field. The gradient of $q_i$ and $t_i$ should be the same, $UDF(q_i) -UDF(t_i) = \|s_i\|$.}
  \label{fig:reg2}
\end{figure}

==> figures/scan_result2.tex <==
\begin{figure*} 
\centering
  \includegraphics[width=2\columnwidth]{figures/images/scan_result2.pdf}
  \caption{Visualized results of our method and NDF\cite{2020ndf}, CAP\cite{capudf} and GIFS\cite{gifs}.}
  \label{fig:scan_result2}
\end{figure*}

==> figures/scan_result3.tex <==
\begin{figure*} 
\centering
  \includegraphics[width=2\columnwidth]{figures/images/scan_result3.pdf}
  \caption{Visualized results of our method and NDF\cite{2020ndf}, CAP\cite{capudf} and GIFS\cite{gifs}.}
  \label{fig:scan_result3}
\end{figure*}

==> figures/shapenet_result3.tex <==
\begin{figure*} 
\centering
  \includegraphics[width=2\columnwidth]{figures/images/shapenet_result3.pdf}
  \caption{Visualized results of our method and state-of-the-art alternatives. Note that we provide the ground-truth normal as input for PSR as it requires. The color map in the figure is the error distribution of the reconstruction. Blue indicates low reconstruction error while yellow indicates higher error values. (S) mean supervised method and (U) means unsupervised method. Methods are ConvOcc\cite{2020Convolutional}, Onet\cite{2019Occupancy}, NP\cite{2020npull}, CAP\cite{capudf}, GIFS\cite{gifs}.}
  \label{fig:shapenet_result3}
\end{figure*}
